Benchmarking Deep Learning Fuzzers

In this work, we set out to conduct the first ground-truth empirical evaluation of state-of-the-art DL fuzzers. Specifically, we first manually created an extensive DL bug benchmark dataset, which includes 627 real-world DL bugs from TensorFlow and PyTorch libraries reported by users between 2020 and 2022. Then we run three state-of-the-art DL fuzzers, i.e., FreeFuzz, DeepRel, and DocTer, on the benchmark by following their instructions. We find that these fuzzers are unable to detect many real bugs collected in our benchmark dataset. Specifically, most (235) of the 257 applicable bugs cannot be detected by any fuzzer. Our systematic analysis further identifies four major, broad, and common factors that affect these fuzzers' ability to detect real bugs. These findings present opportunities to improve the performance of the fuzzers in future work. As a proof of concept, we propose a lightweight corner case generator as an extension to the three DL fuzzers, which simply covers several boundary values as well as DL-specific data types. It helps FreeFuzz, DeepRel, and DocTer detect 12, 12, and 14 more bugs, respectively, that were overlooked by the original fuzzers. Overall, this work complements prior studies on DL fuzzers with an extensive performance evaluation and provides a benchmark for future DL library fuzzing studies. Also, our proposed corner case generator proves that the fuzzers can be extended to detect more bugs by extending their internal fuzzing logic based on the insights provided in root cause analysis.

==> figures/missapiexamples.tex <==
\begin{figure}[t!]
\centering
    \begin{lstlisting} 
import torch
def fn(input):
    dim = -1
    dtype = torch.complex128
    fn_res = torch.cumprod(input, dim, 
    dtype=dtype)
    return fn_res
input = torch.rand([5, 5, 5], 
dtype=torch.float64, requires_grad=True)
fn(input).sum().backward()
    \end{lstlisting} 
  \caption{An example of \textit{Runtime Error} in PyTorch library occured when if the data type of the optional parameter is different with the input tensor.}
\label{fig:issue2}
\end{figure}

==> figures/oracleexamples.tex <==
\begin{figure}[h]
\centering
    \begin{lstlisting} 
...
for d in dimensions:
    for ch in channels:
        ...
        for chann_idx in range(ch):
            single_channel = tensor[...,chann_idx]
            mean = tf.reduce_mean(single_channel)
            print("shape:", single_channel.shape, 
            "channel_idx:",
            chann_idx, "mean:", 
            mean.numpy())
\end{lstlisting} 
\caption{An example of \textit{Inconsistent Results} in TensorFlow library where the output of \textit{tf.reduce\_mean}  is wrong for special tensors with 4 dimensions.}
\label{fig:oracleissue1}
\end{figure}


% \begin{figure}[h]
% \centering
%     \begin{lstlisting} 
%     nFeatures = 52
%     layer_neurons = [nFeatures,128,256,
%     512,256,128,
%     128,64,64,32,32,16,16,8,8]
%     layers = []
%     ...
%     if __name__ == '__main__':
%         process = psutil.Process(os.getpid())
%         tensor = torch.randn(1, nFeatures).cuda()
%         for i in range(2000):
%             m = torch.jit.trace(net, tensor)
%             del m
%             if (i % 200) == 0:
%                 gc.collect()
%                 print(i,  "Memory",
%                 process.memory_info()[0])
% \end{lstlisting} 
% \caption{An example of \textit{Memory Leak} in PyTorch library when using \textit{torch.jit.trace}.}
% \label{fig:oracleissue2}
% \end{figure}

==> figures/rq2_fig.tex <==
\pgfplotsset{width=7cm,compat=1.8}

\begin{figure}[t!]
\centering
\renewcommand{\arraystretch}{1}
\resizebox{1.01\columnwidth}{!}{%
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar, axis on top,
        height=5cm, width=13.5cm,
        bar width=0.4cm,
        ymajorgrids, tick align=inside,
        major grid style={draw=white},
        enlarge y limits={value=.1,upper},
        ymin=0, ymax=6,
        axis x line*=bottom,
        axis y line*=right,
        y axis line style={opacity=0},
        tickwidth=0pt,
        enlarge x limits=true,
        legend style={
            at={(0.7,1)},
            anchor=north,
            legend columns=1,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        ylabel={\# of detected bugs}, 
        %xlabel={}, 
        xticklabel style={rotate=25,anchor=east},
        symbolic x coords={
Runtime Error,
Index Error,
Segfault,
Internal Assertion Failure,
Inconsistent Results,
Out of Bound Read,
Crash},
       xtick=data,
       nodes near coords={
        \pgfmathprintnumber[precision=0]{\pgfplotspointmeta}
       }
    ]
\addplot [draw=none, fill=blue!30] coordinates {
(Runtime Error, 5)
(Index Error, 2)
(Segfault, 1)
(Internal Assertion Failure, 1)
(Inconsistent Results, 1)
(Out of Bound Read,0)
(Crash,0)
};
\addplot [draw=none,fill=red!30] coordinates {
(Runtime Error, 4)
(Index Error, 0)
(Segfault, 0)
(Internal Assertion Failure,0)
(Inconsistent Results, 2)
(Out of Bound Read, 1)
(Crash, 1)
   };
\addplot [draw=none,fill=green!30] coordinates {
(Runtime Error, 0)
(Index Error, 0)
(Segfault, 0)
(Internal Assertion Failure, 2)
(Inconsistent Results, 0)
(Out of Bound Read, 0)
(Crash, 2)
   };
    \legend{FreeFuzz, DeepRel, DocTer}
  \end{axis}
  \end{tikzpicture}}
\caption{Distribution of the bug types detected by fuzzers.}
\label{fig:detectedbugdist}
  \end{figure}

==> tables/real_detections.tex <==


\begin{table*}[h]
\centering
\caption{Summary of detected bugs by the fuzzers.}
\song{we can remove this table}
% \renewcommand{\arraystretch}{1}
% 
\setlength{\tabcolsep}{3pt}
%\resizebox{1\textwidth}{!}{
\begin{tabular}{llllr}
\toprule
Tool  & Release & Bug type & API Signature Information \song{explain what's this} \nima{done} & Bug Id \\
\midrule
FreeFuzz  & v1.10.1 & Internal Assertion &  \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.nn.LayerNorm( normalized_shape, eps=1e-05, 
elementwise_affine=True, device=None, dtype=None)
\end{lstlisting}   & 73174      \\
FreeFuzz  & v1.10.1 & Index Error  &  \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.argsort(input, dim=- 1, descending=False, stable=False)
\end{lstlisting}   &  71477      \\
FreeFuzz & v1.10.1 & Index Error &   \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.sort(input, dim=- 1, descending=False, stable=False, *, out=None)
\end{lstlisting}  &  71477      \\
FreeFuzz  & v1.9.0 & Runtime Error & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.nn.functional.batch_norm(input, running_mean,
running_var, weight=None, bias=None, 
training=False, momentum=0.1, eps=1e-05)
\end{lstlisting}   &  65520    \\
FreeFuzz  & v1.10.1 & Runtime Error  & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.logdet(input)
\end{lstlisting}   & 70669        \\
FreeFuzz  & v1.10.1 & Internal Assertion  & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.nn.MultiLabelMarginLoss(size_average=None, 
reduce=None, reduction='mean')
\end{lstlisting}   & 73176       \\
FreeFuzz  & v1.10.1 & Runtime Error  & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.empty_strided(size, stride, *, dtype=None,
layout=None, device=None, requires_grad=False, pin_memory=False)
\end{lstlisting}   & 70397       \\
FreeFuzz  & v1.10.1 & Runtime Error & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.nn.functional.max_unpool2d(input, indices, kernel_size, stride=None,
padding=0, output_size=None)
\end{lstlisting}   & 73154         \\
FreeFuzz  & v2.6.0   & Inconsistent Results & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
tf.nn.weighted_moments(x, axes, frequency_weights,
keepdims=False, name=None)
\end{lstlisting} & 46995       \\
FreeFuzz  & v2.7.0 & Segfault & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
tf.raw_ops.ConcatV2(values, axis, name=None)
\end{lstlisting}   & GHSA-m4hf-j54p-p353        \\
DeepRel   & v1.8.0 & Runtime Error  & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.kron(input, other, *, out=None)
\end{lstlisting}    & 54135     \\
DeepRel   & v1.10.0 & Runtime Error & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.mm(input, mat2, *, out=None) 
\end{lstlisting} & 69665      \\
DeepRel   & v1.10.0 & Crash & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.nn.functional.normalize(input, p=2.0, dim=1, eps=1e-12, out=None)
\end{lstlisting}  & 70100       \\
DeepRel   & v1.10.1 & Inconsistent Results  &  \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.inverse(input, *, out=None)
\end{lstlisting}  & 71084      \\
DeepRel   & v1.10.1 & Inconsistent Results & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.cholesky(input, upper=False, *, out=None)
\end{lstlisting}  & 71084   \\
DeepRel  & v1.10.1 & Runtime Error &  \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.nn.LayerNorm(normalized_shape, eps=1e-05, 
elementwise_affine=True, device=None, dtype=None)
\end{lstlisting}    & 73174      \\
DeepRel  & v1.10.1 & Runtime Error & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.nn.BCELoss(weight=None, size_average=None,
reduce=None, reduction='mean')
\end{lstlisting}   & 72824       \\
DeepRel  & v2.4.0 & Out of Bound Read & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
tf.raw_ops.MatrixTriangularSolve(matrix, rhs, 
lower=True, adjoint=False, name=None)
\end{lstlisting}  & GHSA-vqw6-72r7-fgw7 \\
DocTer   &  v1.7.0  & Crash & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
torch.save(obj, f, pickle_module=pickle,
pickle_protocol=DEFAULT_PROTOCOL, _use_new_zipfile_serialization=True)
\end{lstlisting}  & 47201           \\
DocTer   & v2.4.0 & Internal Assertion & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
tf.strings.substr(input, pos, len,
unit='BYTE', name=None)
\end{lstlisting} & GHSA-mmq6-q8r3-48fm        \\
DocTer   & v2.4.0 & Crash & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
tf.transpose(a, perm=None, 
conjugate=False, name='transpose')
\end{lstlisting} & GHSA-xqfj-cr6q-pc8w        \\
DocTer   & v2.8.0 & Internal Assertion & \begin{lstlisting} [backgroundcolor = \color{white},
                    basicstyle=\small,
                    escapechar=`,
                   language = Python]
tf.strings.unsorted_segment_join(inputs, 
segment_ids, num_segments, separator='', name=None)
\end{lstlisting} & GHSA-hx9q-2mx4-m4pg         \\
\bottomrule
\end{tabular}
\label{tab:detailedTrueBugs}
\end{table*}
